DiGS : Divergence guided shape implicit neural representation for unoriented point clouds

Shape implicit neural representations (INRs) have recently shown to be effective in shape analysis and reconstruction tasks. Existing INRs require point coordinates to learn the implicit level sets of the shape. When a normal vector is available for each point, a higher fidelity representation can be learned, however normal vectors are often not provided as raw data. Furthermore, the method's initialization has been shown to play a crucial role for surface reconstruction. In this paper, we propose a divergence guided shape representation learning approach that does not require normal vectors as input. We show that incorporating a soft constraint on the divergence of the distance function favours smooth solutions that reliably orients gradients to match the unknown normal at each point, in some cases even better than approaches that use ground truth normal vectors directly. Additionally, we introduce a novel geometric initialization method for sinusoidal INRs that further improves convergence to the desired solution. We evaluate the effectiveness of our approach on the task of surface reconstruction and shape space learning and show SOTA performance compared to other unoriented methods. Code and model parameters available at our project page https://chumbyte.github.io/DiGS-Site/.

==> assets/figures/dfaust_qualitative.tex <==
\begin{figure*}
     \centering
     \resizebox{0.9\textwidth}{!}{
     \begin{tabular}{c c c c c | c c c c c}
         \rotatebox[origin=c]{90}{SIREN}
         &
         \raisebox{-.5\height}{\includegraphics[width=0.1\linewidth, trim=250pt 135pt 165pt 110pt, clip]{assets/figures/dfaust/siren0.png} }
         &
         \raisebox{-.5\height}{\includegraphics[width=0.1\linewidth, trim=250pt 135pt 165pt 110pt, clip]{assets/figures/dfaust/siren1.png} }
         &
         \raisebox{-.5\height}{\includegraphics[width=0.1\linewidth, trim=250pt 135pt 165pt 110pt, clip]{assets/figures/dfaust/siren9.png} }
         &
         \raisebox{-.5\height}{\includegraphics[width=0.1\linewidth, trim=250pt 135pt 165pt 110pt, clip]{assets/figures/dfaust/siren29.png} }
         &
         \rotatebox[origin=c]{90}{SIREN wo n}
         &
         \raisebox{-.5\height}{\includegraphics[width=0.1\linewidth, trim=250pt 135pt 165pt 110pt, clip]{assets/figures/dfaust/siren-wo-n-0.png} }
         &
         \raisebox{-.5\height}{\includegraphics[width=0.1\linewidth, trim=250pt 135pt 165pt 110pt, clip]{assets/figures/dfaust/siren-wo-n-1.png}} 
         &
         \raisebox{-.5\height}{\includegraphics[width=0.1\linewidth, trim=250pt 135pt 165pt 110pt, clip]{assets/figures/dfaust/siren-wo-n-9.png}} 
         &
         \raisebox{-.5\height}{\includegraphics[width=0.1\linewidth, trim=250pt 135pt 165pt 110pt, clip]{assets/figures/dfaust/siren-wo-n-29.png}} 
         \\
         $d_C$, $d_{\vec{C}}$& 8.62, 6.49 & 6.91, 3.15 & 3.58, 0.86 & 6.66, 0.74 && 18.52, 17.26 & 15.17, 14.05 & 4.89, 1.60 & 3.14, 1.37\\
        %  \rule{0pt}{-0.05ex} &&&& \\  
         \rotatebox[origin=c]{90}{IGR}
         &
         \raisebox{-.5\height}{\includegraphics[width=0.1\linewidth, trim=250pt 135pt 165pt 110pt, clip]{assets/figures/dfaust/igr0.png} }
         &
         \raisebox{-.5\height}{\includegraphics[width=0.1\linewidth, trim=250pt 135pt 165pt 110pt, clip]{assets/figures/dfaust/igr1.png} }
         &
         \raisebox{-.5\height}{\includegraphics[width=0.1\linewidth, trim=250pt 135pt 165pt 110pt, clip]{assets/figures/dfaust/igr9.png} }
         &
         \raisebox{-.5\height}{\includegraphics[width=0.1\linewidth, trim=250pt 135pt 165pt 110pt, clip]{assets/figures/dfaust/igr29.png} }
         &
         \rotatebox[origin=c]{90}{IGR wo n}
         &
         \raisebox{-.5\height}{\includegraphics[width=0.1\linewidth, trim=250pt 135pt 165pt 110pt, clip]{assets/figures/dfaust/igr-wo-normals-0.png} }
         &
         \raisebox{-.5\height}{\includegraphics[width=0.1\linewidth, trim=250pt 135pt 165pt 110pt, clip]{assets/figures/dfaust/igr-wo-normals-1.png}} 
         &
         \raisebox{-.5\height}{\includegraphics[width=0.1\linewidth, trim=250pt 135pt 165pt 110pt, clip]{assets/figures/dfaust/igr-wo-normals-9.png}} 
         &
         \raisebox{-.5\height}{\includegraphics[width=0.1\linewidth, trim=250pt 135pt 165pt 110pt, clip]{assets/figures/dfaust/igr-wo-normals-29.png}} 
         \\
         $d_C$, $d_{\vec{C}}$& 8.58, 14.31 & 4.10, 4.61 & 0.80, 0.84 & 1.33, 1.36 && 25.19, 37.13 & 4.62, 5.51 & 1.81, 1.73 & 1.18, 1.16\\
        %  \rule{0pt}{0.05ex} &&&& \\         
         
         \rotatebox[origin=c]{90}{DiGS+n}
         &
         \raisebox{-.5\height}{\includegraphics[width=0.1\linewidth, trim=250pt 135pt 165pt 110pt, clip]{assets/figures/dfaust/DiGS-w-normals-0.png} }
         &
         \raisebox{-.5\height}{\includegraphics[width=0.1\linewidth, trim=250pt 135pt 165pt 110pt, clip]{assets/figures/dfaust/DiGS-w-normals-1.png} }
         &
         \raisebox{-.5\height}{\includegraphics[width=0.1\linewidth, trim=250pt 135pt 165pt 110pt, clip]{assets/figures/dfaust/DiGS-w-normals-9.png} }
         &
         \raisebox{-.5\height}{\includegraphics[width=0.1\linewidth, trim=250pt 135pt 165pt 110pt, clip]{assets/figures/dfaust/DiGS-w-normals-29.png}}   
         &   
         \rotatebox[origin=c]{90}{DiGS}
         &
         \raisebox{-.5\height}{\includegraphics[width=0.1\linewidth, trim=250pt 135pt 165pt 110pt, clip]{assets/figures/dfaust/DiGS-wo-normals-0.png} }
         &
         \raisebox{-.5\height}{\includegraphics[width=0.1\linewidth, trim=250pt 135pt 165pt 110pt, clip]{assets/figures/dfaust/DiGS-wo-normals-1.png} }
         &
         \raisebox{-.5\height}{\includegraphics[width=0.1\linewidth, trim=250pt 135pt 165pt 110pt, clip]{assets/figures/dfaust/DiGS-wo-normals-9.png} }
         &
         \raisebox{-.5\height}{\includegraphics[width=0.1\linewidth, trim=250pt 135pt 165pt 110pt, clip]{assets/figures/dfaust/DiGS-wo-normals-29.png}} \\
         $d_C$, $d_{\vec{C}}$ & 1.02, 1.12 & 0.91, 0.99 & 0.72, 0.69 & 1.06, 0.64 && 8.24, 1.23 & 4.27, 1.00 & 3.28, 0.81 & 2.70, 0.78\\
        % \rotatebox[origin=c]{90}{$#$ iterations}
         \# iters
         &6000  &  12000  & 60000  & 180000  & &6000  &  12000  & 60000  & 180000 Its \\
        \rotatebox[origin=c]{90}{}
         &\multicolumn{4}{c}{With Normals}& &\multicolumn{4}{c}{Without Normals} \\
     \end{tabular}}
        \caption{Qualitative surface reconstruction results on the DFaust \cite{bogo2017dynamic} dataset. Each column show the zero level set at progressing training iterations. Two- and one-sided Chamfer distances are also given. ``+n" and ``wo n" refer to with and without ground truth normal supervision respectively.}
        \label{fig:dfaust_comparisons}
\end{figure*}

==> assets/figures/surface_reconstruction_pod_graphs.tex <==
\begin{figure}
     \centering
     \begin{tabular}{c c c }
                 \includegraphics[width=0.29\linewidth]{assets/figures/surface_recon/pod_graphs/anchor_pod_results.png}
                 &
                 \includegraphics[width=0.29\linewidth]{assets/figures/surface_recon/pod_graphs/daratech_pod_results.png} 
                 &
                 \includegraphics[width=0.29\linewidth]{assets/figures/surface_recon/pod_graphs/dc_pod_results.png} \\
                 
                  \includegraphics[width=0.29\linewidth]{assets/figures/surface_recon/pod_graphs/gargoyle_pod_results.png}
                 &
                 \includegraphics[width=0.29\linewidth]{assets/figures/surface_recon/pod_graphs/lord_quas_pod_results.png} 
                 &
                 \includegraphics[width=0.29\linewidth]{assets/figures/surface_recon/pod_graphs/mean_pod_results.png} \\
                 
     \end{tabular}
        \caption{Quantitative evaluation of surface reconstruction using the Percentage of Distance metric. }
        \label{fig:surface_recon_pods_results}
\end{figure}

==> assets/tables/surface_reconstruction_SRB_summary_all.tex <==
\begin{table}[]\scriptsize
    \centering
    \begin{tabular}{l c c c c}
         \toprule
          Method    & $d_{C}$ & $d_H$ & $d_{C}$ dev. & $d_{H}$ dev  \\
            \hline
            DGP             & 0.21 & 5.18 & 0.05 & 2.78 \\
            IGR             & 0.19 & 2.99 & 0.03 & 0.59 \\
            SIREN           & 0.19 & 3.86 & 0.03 & 1.46 \\
            NSP             & 0.17 & 2.85 & 0.01 & 0.44 \\
            PHASE           & \textbf{0.16} & \textbf{2.77} & \textbf{0.00} & \textbf{0.36} \\
            DiGS w n        & 0.18 & 3.55 & 0.02 & 1.15 \\
            % DiGS + sqrt     & 0.19 & 3.24 \\
            \hline
            IGR wo n        & 1.38 & 16.33 & 1.20 & 12.59 \\
            SIREN wo n      & 0.42 & 7.67  & 0.23 & 3.93  \\
            SAL             & 0.36 & 7.47  & 0.18 & 3.74  \\
            IGR+FF          & 0.96 & 11.06 & 0.78 & 7.33  \\
            PHASE+FF        & 0.22 & 4.96  & 0.04 & 1.23  \\
            DIGS            & \textbf{0.19} & \textbf{3.85}  & \textbf{0.01} & \textbf{0.11}  \\
            % DiGS + Sqrt     & 0.20 & 4.92  \\
            % + Uniform sampl & 0.19 & 3.52  \\
         \bottomrule
    \end{tabular}
    \caption{Results on the Surface Reconstruction Benchmark. Methods above the line use ground truth normal information, and methods below do not. We report the mean Chamfer $d_{C}$ and Hausdorff distance $d_H$ to the ground truth scans, but as the models differ greatly in difficulty, we also report the mean deviation of these metrics from the best performing method for each shape ($d_{C}$ dev. and $d_{H}$ dev.).}
    \label{tab:results:surf-recon-summary-all}
\end{table}

==> assets/tables/surface_reconstruction_results.tex <==
\begin{table*}[]\scriptsize
    \centering
    \begin{tabular}{l c c c c c c | c c }
         \toprule
          & & & \multicolumn{2}{c}{GT} & \multicolumn{2}{c}{Scans}  & &  \\
          & & Method & $d_{C}$ & $d_H$ & $d_{\vec{C}}$ & $d_{\vec{H}}$  
          & mLCV$_{k=10}$ & mLCV$_{k=50}$ \\
            \hline
            
            \multirow{6}{*}{anchor} &\multirow{4}{*}{with n} & DGP & 0.33 & 8.82 & 0.08 & 2.79 & 2.2 & 3.88 \\ 
                                     && IGR & 0.23 & 4.71 & 0.12 & 1.32 & 0.74 & 2.63 \\ 
                                     && PHASE & \textbf{0.21} & \textbf{4.29} & 0.09 & 1.23 & - & - \\
                                     && FFN & 0.31 & 4.49 & 0.10 & 0.10 & - & - \\
                                     && NSP & 0.22 & 4.65 & 0.11 & 1.11 & - & - \\
                                     && SIREN & 0.31 & 7.32 & 0.11 & 1.23 & 0.55 & 2.22 \\ 
                                     && DiGS w n & 0.28 & 5.71 & 0.11 & 1.14 & \textbf{0.52} &\textbf{ 2.05} \\ 

                                       \cline{2-9}    
                               &\multirow{3}{*}{w/o n}& SIREN wo n & 0.72 & 10.98 & 0.11 & 1.27 & 2.43 & 11.71 \\ 
                                     && IGR wo n & 0.45 & 7.45 & 0.17 & 4.55 & 0.98 & 4.54 \\ 
                                     && DiGS (Ours)& \textbf{0.31} & \textbf{7.20} & 0.11 & \textbf{1.15} &\textbf{ 0.63} & \textbf{2.58} \\ 
            \hline
            \multirow{6}{*}{gargoyle}    &\multirow{4}{*}{with n}& DGP & 0.21 & 5.98 & \textbf{0.06} & 3.41 & 2.44 & 4.65 \\ 
                                         && IGR & 0.18 & \textbf{2.85} & 0.1 & 1.29 & 1.0 & 2.85 \\ 
                                         && PHASE & \textbf{0.16} & 3.14 & 0.07 & 1.09 & - & - \\
                                         && FFN & 0.22 & 5.04 & 0.09 & 0.09 & - & - \\
                                         && NSP & 0.16& 3.2 & 0.08 & 2.75 & - & - \\
                                         && SIREN & 0.17 & 4.26 & 0.09 & \textbf{0.82} & \textbf{0.55} & \textbf{1.65} \\ 
                                         && DiGS w n & \textbf{ 0.16} & 3.81 & 0.09 & 0.90 & \textbf{0.55} & 1.66 \\ 
                                           \cline{2-9}    
                               &\multirow{3}{*}{w/o n}& SIREN wo n & 0.46 & 7.76 & \textbf{0.08} &\textbf{ 0.68} & 2.16 & 9.8 \\ 
                                         && IGR wo n & 0.77 & 17.46 & 0.18 & 2.04 & 2.72 & 12.27 \\ 
                                         && DiGS (Ours)& \textbf{0.16} & \textbf{4.25} & 0.09 & 0.82 & \textbf{0.58} & \textbf{1.77} \\ 
            \hline
            \multirow{6}{*}{lord quas}   &\multirow{4}{*}{with n}& DGP & 0.14 & 3.67 & 0.04 & 2.03 & 2.2 & 3.83 \\ 
                                         && IGR & 0.12 & 1.17 & 0.07 & 0.98 & 0.87 & 2.01 \\
                                         && PHASE & \textbf{0.11} & 0.96 & 0.04 & 0.96 & - & - \\
                                         && FFN & 0.35 & 3.90 & 0.06 & 0.06 & - & - \\
                                         && NSP & 0.12 & 0.69  & 0.05 & 0.62 & - & - \\
                                         && SIREN & 0.12 & \textbf{0.62} & 0.08 & 0.81 & \textbf{0.37} & \textbf{0.82} \\ 
                                        & & DiGS w n & 0.12 & 1.1 & 0.06 & 0.77 & \textbf{0.37} & 0.86 \\ 
                                           \cline{2-9}    
                               &\multirow{3}{*}{w/o n}& SIREN wo n & 0.35 & 8.96 & 0.06 & \textbf{0.65} & 1.54 & 7.05 \\ 
                                         && IGR wo n & 0.16 & 4.22 & 0.08 & 1.14 & 0.63 & 2.14 \\ 
                                         && DiGS (Ours)& \textbf{0.12} & \textbf{1.27} & 0.06 & 0.69 & \textbf{0.38} & \textbf{0.89} \\ 
            \hline
            \multirow{6}{*}{daratech}    &\multirow{4}{*}{with n}& DGP & 0.20 & 3.14 & \textbf{0.04} & 1.89 & 3.83 & 8.36 \\ 
                                         && IGR & 0.25 & 4.01 & 0.14 & 1.59 & 1.16 & 4.64 \\ 
                                         && PHASE & \textbf{0.18} & \textbf{2.92} & 0.08 & 1.8 & - & - \\
                                         && FFN & 0.34 & 5.97 & 0.10 & 0.10 & - & - \\
                                         && NSP & 0.21  & 4.35  & 0.08 & 1.14 & - & - \\
                                         && SIREN & 0.21 & 4.74 & 0.09 & 1.85 & 1.01 & 4.01 \\ 
                                         && DiGS w n & 0.21 & 5.02 & 0.09 & \textbf{1.75} & 1.0 & 3.96 \\ 
                                           \cline{2-9}    
                               &\multirow{3}{*}{w/o n}& SIREN wo n & 0.21 & 4.37 & 0.09 & 1.78 & \textbf{0.97} & \textbf{3.76} \\ 
                                         && IGR wo n & 4.9 & 42.15 & 0.7 & 3.68 & 5.85 & 30.17 \\ 
                                         && DiGS (Ours)& 0.21 & \textbf{4.22} & 0.09 & \textbf{1.75} & 1.00 & 3.96 \\ 
            \hline
            \multirow{6}{*}{dc} &\multirow{4}{*}{with n} & DGP & 0.18 & 4.31 &\textbf{ 0.04} & \textbf{2.53} & 2.81 & 5.41 \\ 
                                 && IGR & 0.17 & 2.22 & 0.09 & 2.61 & 1.05 & 2.76 \\ 
                                 && PHASE & 0.15 & 2.52 & 0.05 & 2.78 & - & - \\
                                 && FFN & 0.20 & 2.87 & 0.10 & 0.12 & - & - \\
                                 && NSP & \textbf{0.14} & \textbf{1.35} & 0.06 & 2.75 & - & - \\
                                 && SIREN & 0.15 & 2.37 & 0.07 & 2.71 & 0.50 & 1.29 \\ 
                                 && DiGS w n & 0.15 & 2.13 & 0.06 & 2.74 & 0.50 & \textbf{1.26} \\ 
                                 \cline{2-9}    
                               &\multirow{3}{*}{w/o n}  & SIREN wo n & 0.34 & 6.27 & \textbf{0.06} & \textbf{2.71} & 1.75 & 7.69 \\ 
                                & & IGR wo n & 0.63 & 10.35 & 0.14 & 3.44 & 2.79 & 13.0 \\ 
                                & & DiGS (Ours)& \textbf{0.15} & \textbf{2.29} & 0.07 & 2.72 & \textbf{0.50} & \textbf{1.27} \\ 


         \bottomrule
    \end{tabular}
    \caption{Results on the Surface Reconstruction Benchmark using Chamfer $d_{C}$, Hausdorff distance $d_H$ and the proposed mean Local Chamfer Variance (mLCV) with 10 and 50 neighbors. We compare to methods with and without normal vectors as ground truth during training.  The \textit{scans} column reports the one sided distances ($d_{\vec{C}}, d_{\vec{H}}$) between the reconstruction and the simulated scans which give a measure of the reconstruction's overfit to the noisy input. }
    \label{tab:results:surface reconstructon_all}
\end{table*}
% \begin{table}[]\scriptsize
%     \centering
%     \begin{tabular}{l c c c c c c}
%          \toprule
%           & & \multicolumn{2}{c}{GT} & \multicolumn{2}{c}{Scans} \\
%           & Method & $d_{C}$ & $d_H$ & $d_{\vec{C}}$ & $d_{\vec{H}}$ \\
%             \hline
%             \multirow{4}{*}{Anchor}    & DGP   & 0.33 & 8.82 & 0.08 & 2.79 \\ 
%                                       & IGR   & 0.22 & 4.71 & 0.12 & 1.32 \\
%                                       & NS    & 0.22 & 4.65 & 0.11 & 1.11 \\
%                                       & SIREN & 0.27 & 6.18 & 0.13 & 1.88 \\
%                                       & SIREN - ours & 0.32 & 7.65 & 0.13 & 1.16 \\
%                                       & SIREN wo n & 0.56 & 10.94 & 0.12 & 1.22  \\
%                                       & \textbf{Ours}&&&& \\
%             \hline
%             \multirow{4}{*}{Daratech}  & DGP   & 0.2 & 3.14 & 0.04 & 1.89 \\ 
%                                     %   & IGR   & 0.25 & 4.01 & 0.08 & 1.59 \\ % reported values
%                                       & IGR   & 0.25 & 4.01 & 1.14 & 1.59 \\  % reproduced values
%                                       &NS     & 0.21 & 4.35 & 0.08 & 1.14 \\
%                                       & SIREN & 0.29 & 4.46 & 0.12 & 1.65 \\                                       
%                                       &SIREN - ours & 0.22 & 4.4 & 0.11 & 1.24 \\
%                                       & SIREN wo n & 0.24 & 4.68 & 0.11 & 0.96  \\
%                                       &\textbf{Ours}&&&&\\
%             \hline
%             \multirow{4}{*}{DC}         & DGP   & 0.18 & 4.31 & 0.04 & 2.53 \\ 
%                                         & IGR   & 0.17 & 2.22 & 0.09 & 2.61 \\
%                                         & NS    & 0.14 & 1.35 & 0.06 & 2.75 \\
%                                         & SIREN & 0.18 & 2.27 & 0.09 & 1.92 \\                                        
%                                         & SIREN - ours & 0.16 & 2.42 & 0.08 & 2.69 \\
%                                         & SIREN wo n & 0.31 & 5.70 & 0.08 & 2.72 \\
%                                         & \textbf{Ours}&&&&\\
%             \hline
%             \multirow{4}{*}{Gargoyle}   & DGP   & 0.21 & 5.98 & 0.06 & 3.41 \\ 
%                                         % & IGR   & 0.16 & 3.52 & 0.06 & 3.41 \\  %reported values
%                                         & IGR   & 0.18 & 2.85  & 0.10 & 1.29 \\ % reproduced values
%                                         & NS    & 0.16 & 3.20 & 0.08 & 2.75 \\
%                                         & SIREN & 0.29 & 3.90 & 0.13 & 1.93 \\                                        
%                                         & SIREN - ours & 0.17 & 4.50 & 0.10 & 0.77 \\
%                                         & SIREN wo n &  0.4 & 9.18 & 0.10 & 0.96 \\
%                                         & \textbf{Ours}&&&&\\
%             \hline
%             \multirow{4}{*}{Lord Quas}  & DGP   & 0.14 & 3.67 & 0.04 & 2.03 \\ 
%                                         & IGR   & 0.12 & 1.17 & 0.07 & 0.98 \\
%                                         & NS    & 0.12 & 0.69 & 0.05 & 0.62\\
%                                         & SIREN & 0.13 & 0.89 & 0.06 & 0.96 \\                                        
%                                         & SIREN - ours & 0.13 & 0.74 & 0.09 & 0.91 \\
%                                         & SIREN wo n & 0.26 & 8.49 & 0.09 & 1.38 \\
%                                         & \textbf{Ours}&&&&\\
%          \bottomrule
%     \end{tabular}
%     \caption{Results on the Surface Reconstruction Benchmark using the Chamfer $d_{C}$ and Hausdorff distance $d_H$. The \textit{scans} column reports the one sided distances ($d_{\vec{C}}, d_{\vec{H}}$) between the reconstruction and the simulated scans which give a measure of the reconstruction's overfit to the noisy input. }
%     \label{tab:results:surface reconstructon}
% \end{table}

==> assets/tables/surface_reconstruction_results_wo_n.tex <==
\begin{table}[t]\scriptsize
    \centering
    \setlength\tabcolsep{3.0pt} % default value: 6pt
    \begin{tabular}{l c c c c c | c c }
         \toprule
          & & \multicolumn{2}{c}{GT} & \multicolumn{2}{c}{Scans}  & &  \\
          & Method & $d_{C}$ & $d_H$ & $d_{\vec{C}}$ & $d_{\vec{H}}$  
          & $mLCV_{10}$ & $mLCV_{50}$ \\
            \hline
            
            \multirow{3}{*}{anchor}  & SAL & 0.42 & 7.21 & 0.17 & 4.67 & 0.86 & 3.87 \\
                               &SIREN wo n & 0.72 & 10.98 & 0.11 & 1.27 & 2.43 & 11.71 \\ 
                                     & IGR wo n & 0.45 & 7.45 & 0.17 & 4.55 & 0.98 & 4.54 \\ 
                                     & DiGS (Ours)& \textbf{0.31} & \textbf{7.20} & 0.11 & \textbf{1.15} &\textbf{ 0.63} & \textbf{2.58} \\ 
            \hline
            \multirow{3}{*}{gargoyle}  & SAL & 0.45 & 9.74 & 0.21 & 3.84 & 3.6 & 16.09 \\  
                               & SIREN wo n & 0.46 & 7.76 & \textbf{0.08} &\textbf{ 0.68} & 2.16 & 9.8 \\ 
                                         & IGR wo n & 0.77 & 17.46 & 0.18 & 2.04 & 2.72 & 12.27 \\ 
                                         & DiGS (Ours)& \textbf{0.16} & \textbf{4.25} & 0.09 & 0.82 & \textbf{0.58} & \textbf{1.77} \\ 
            \hline
            \multirow{3}{*}{lord quas} & SAL & 0.13 & 4.14 & 0.07 & 4.04 & 0.44 & 1.2 \\
                              & SIREN wo n & 0.35 & 8.96 & 0.06 & \textbf{0.65} & 1.54 & 7.05 \\ 
                                         & IGR wo n & 0.16 & 4.22 & 0.08 & 1.14 & 0.63 & 2.14 \\ 
                                         & DiGS (Ours)& \textbf{0.12} & \textbf{1.27} & 0.06 & 0.69 & \textbf{0.38} & \textbf{0.89} \\ 
            \hline
            \multirow{3}{*}{daratech}   & SAL & 0.62 & 13.21 & 0.11 & 2.15 & 3.11 & 14.97 \\ 
                              & SIREN wo n & \textbf{0.21} & 4.37 & \textbf{0.09} & 1.78 & \textbf{0.97} & \textbf{3.76} \\ 
                                         & IGR wo n & 4.9 & 42.15 & 0.7 & 3.68 & 5.85 & 30.17 \\ 
                                         & DiGS (Ours)& \textbf{0.21} & \textbf{4.22} & \textbf{0.09} & \textbf{1.75} & 1.00 & 3.96 \\ 
            \hline
            \multirow{3}{*}{dc} & SAL & 0.18 & 3.06 & 0.08 & 2.82 & 0.78 & 2.55 \\
                                & SIREN wo n & 0.34 & 6.27 & \textbf{0.06} & \textbf{2.71} & 1.75 & 7.69 \\ 
                                & IGR wo n & 0.63 & 10.35 & 0.14 & 3.44 & 2.79 & 13.0 \\ 
                                & DiGS (Ours)& \textbf{0.15} & \textbf{2.29} & 0.07 & 2.72 & \textbf{0.50} & \textbf{1.27} \\ 


         \bottomrule
    \end{tabular}
    \caption{Results on the Surface Reconstruction Benchmark using Chamfer $d_{C}$, Hausdorff distance $d_H$ and the proposed mean Local Chamfer Variance (mLCV) with 10 and 50 neighbors. We compare to methods with and without normal vectors as ground truth during training.  The \textit{scans} column reports the one sided distances ($d_{\vec{C}}, d_{\vec{H}}$) between the reconstruction and the simulated scans which give a measure of the reconstruction's overfit to the noisy input. }
    \label{tab:results:surface reconstructon}
\end{table}


==> sections/checklist.tex <==
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See \secref{Sec:results}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{see \secref{Sec:broader_impact}}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{See supplemental material}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See \secref{Sec:intro}}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See \secref{Sec:results} and supplemental material}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{Error bars are not reported because it would be too computationally expensive}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See supplemental material}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNo{There is no particular named license associated with the data, however, they are freely available for use for academic purposes on the author's website.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{Code is provided as a URL (redacted for submission)}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{See \secref{Sec:results}}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{Inapplicable for the datasets used in the scope of this paper.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{No crowdsourcing or human subjects in the work}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{No crowdsourcing or human subjects in the work}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{No crowdsourcing or human subjects in the work}
\end{enumerate}

\end{enumerate}
